LingMess: Linguistically Informed Multi Expert Scorers for Coreference Resolution

While coreference resolution typically involves various linguistic challenges, recent models are based on a single pairwise scorer for all types of pairs. We present LingMess, a new coreference model that defines different categories of coreference cases and optimize multiple pairwise scorers, where each scorer learns a specific set of linguistic challenges. Our model substantially improves pairwise scores for most categories and outperforms cluster-level performance on Ontonotes and 5 additional datasets. Our model is available in https://github.com/shon-otmazgin/lingmess-coref

==> 02_background.tex <==
\section{Background: the s2e Model}
\label{sec:bg}

The \emph{s2e} model~\citep{kirstain-etal-2021-coreference} is a lightweight and efficient coreference model, which avoids the costly construction of full-fledged span representations, by considering only span boundaries. This model achieves the current best coreference scores among all practical models.\footnote{The CorefQA model~\citep{wu-etal-2020-corefqa} achieves a substantially higher score, but requires to run a separate BERT inference for each mention, making it highly impractical. }

Given a sequence of tokens $x_1, ..., x_n$, each span is represented by its start/end tokens. For a pair of spans $c=(x_i, x_j)$, $q=(x_k, x_\ell)$ where $c$ (``candidate'') appears before $q$ (``query''), a parameterized function $f_m(c)$ ($f_m(q)$) scores how fit a given span is to be a mention, while a parameterized function $f_a(c,q)$ scores how fit $c$ is to be a coreferring antecedent of $q$ (As computing antecedent scores for all possible pairs would result in a complexity of $\mathcal{O}(n^4)$, in practice only the highest scoring spans according to $f_m$ are fed to the antecedent scorer $f_a$).
These functions operate over contextualized vector representations, obtained by a BERT-like model. For the exact function form, see Appendix~\ref{app:s2e}.

Finally, the final pairwise score $F_\textsc{g}(c, q)$ is composed of the two mention scores $f_m(q)$, $f_m(c)$ and the antecedent score $f_a(c, q)$. 

\begin{align*}
F_{\textsc{g}}(c, q) = 
\begin{cases}
f_m(c) + f_m(q) + f_a(c, q) & c \neq \varepsilon \\
0 & c = \varepsilon %\numberthis \label{eq:f_g}
\end{cases}
\end{align*}
where $\varepsilon$ is the null antecedent.

For each possible mention $q$, the learning objective optimizes the sum of probabilities over the true antecedent $\hat{c}$ of $q$:
\begin{align*}
L_{\textsc{g}}(q) = \log \sum_{\hat{c} \in \mathcal{C}(q) \cap \textsc{gold}(q)}P_{\textsc{g}}(\hat{c} \mid q) 
\end{align*}
where $\mathcal{C}(q)$ is the set of all candidate antecedents\footnote{All spans before $q$ that passed some pruning threshold.} with a null antecedent $\varepsilon$. $\textsc{gold}(q)$ is the set of the true antecedents of $q$.
$P_\textsc{g}(c \mid q)$ is computed as a softmax over $F_\textsc{g}(c, q)$ scores for $c$ values in $\mathcal{C}(q)$:
\begin{align*}
P_{\textsc{g}}(\hat{c} \mid q) = \frac{\exp{F_\textsc{g}(\hat{c}, q)}}{\sum\limits_{c' \in \mathcal{C}(q)} \exp{F_\textsc{g}(c', q)}} %\numberthis \label{eq:p_g}
\end{align*}


